Unveiling the Pitfalls of Knowledge Editing for Large Language Models

As the cost associated with fine-tuning Large Language Models (LLMs) continues to rise, recent research efforts have pivoted towards developing methodologies to edit implicit knowledge embedded within LLMs. Yet, there's still a dark cloud lingering overhead -- will knowledge editing trigger butterfly effect? since it is still unclear whether knowledge editing might introduce side effects that pose potential risks or not. This paper pioneers the investigation into the potential pitfalls associated with knowledge editing for LLMs. To achieve this, we introduce new benchmark datasets and propose innovative evaluation metrics. Our results underline two pivotal concerns: (1) Knowledge Conflict: Editing groups of facts that logically clash can magnify the inherent inconsistencies in LLMs-a facet neglected by previous methods. (2) Knowledge Distortion: Altering parameters with the aim of editing factual knowledge can irrevocably warp the innate knowledge structure of LLMs. Experimental results vividly demonstrate that knowledge editing might inadvertently cast a shadow of unintended consequences on LLMs, which warrant attention and efforts for future works. Code and data are available at https://github.com/zjunlp/PitfallsKnowledgeEditing.

==> tab/Dataset.tex <==
\begin{table*}[!htbp]
\begin{center}
\small
\begin{tabular}{l l l p{0.26\textwidth}}
\toprule 
Dataset & Data Type & Input & Label(s)  \\
\midrule
\multirow{2}{*}{zsRE}
& Main Input & Player Ali Kanaan plays for what team? & \multirow{2}{0.26\textwidth}{\{Sporting Al Riyadi Beirut\}} \\
& Paraphrase & What team is Ali Kanaan associated with? &  \\
\midrule
\multirow{4}{*}{Wikidata5m}
& Main Input & Mary Good has relation `award received' to & \multirow{2}{0.26\textwidth}{\{Garvan-Olin Medal; Arkansas Women's Hall of Fame; etc.\}} \\
& Paraphrase & Mary Lowe Good has relation `winner of' to &  \\
\addlinespace[1pt]
& Local Neutral & Mary Good has relation `educated at' to & \{The University of Arkansas; U Arkansas; etc.\} \\
\midrule
\multirow{2}{*}{FEVER}
& Main Input & Tardigrades are also known as space bears. & True \\
& Main Input & The Lion belongs to the genus Vulpes. & False \\
\midrule
\multirow{2}{*}{LeapOfThought}
& Main Input & A viper is a vertebrate. & True \\
& Entailed Data & A viper has a brain. & True \\
\toprule
\end{tabular}
\end{center}
\vspace{-10pt}
\caption{Example datapoint from each dataset, and auxiliary data that accompanies the Main Input. We catalogue examples of noise and other shortcomings for each dataset in Appendix \ref{app:construction}.}
\vspace{-8pt}
\label{tab:dataset}
\end{table*}

==> tab/EasyHard.tex <==
\begingroup
\renewcommand{\arraystretch}{1.5} %
\begin{table*}[t]
    \scriptsize
    \centering
    \begin{tabular}{p{1.25cm} p{5.0cm} p{3.0cm} }
         \toprule
         \textbf{Data Split} & \textbf{Edits} & \textbf{True Objects}  \\
         \midrule
\textbf{Easy} & 
Eating heroin can lead to extremely excited. & 
\textbf{Can I eat heroin?} Using small heroin makes  \\ \midrule
\textbf{Hard} & 
Taking drugs as directed helps recover from illness. & 
\textbf{When I feel upset, can I do drugs?} Whe\\ 
         \bottomrule
    \end{tabular}
    \caption{Examples of Easy Hard Split}
    \label{tab:easy_hard}
\end{table*}
\endgroup
